Neural Collapse in Multi-label Learning with Pick-all-label Loss

We study deep neural networks for the multi-label classification (MLab) task through the lens of neural collapse (NC). Previous works have been restricted to the multi-class classification setting and discovered a prevalent NC phenomenon comprising of the following properties for the last-layer features: (i) the variability of features within every class collapses to zero, (ii) the set of feature means form an equi-angular tight frame (ETF), and (iii) the last layer classifiers collapse to the feature mean upon some scaling. We generalize the study to multi-label learning, and prove for the first time that a generalized NC phenomenon holds with the "pick-all-label" formulation, which we term as MLab NC. While the ETF geometry remains consistent for features with a single label, multi-label scenarios introduce a unique combinatorial aspect we term the "tag-wise average" property, where the means of features with multiple labels are the scaled averages of means for single-label instances. Theoretically, under proper assumptions on the features, we establish that the only global optimizer of the pick-all-label cross-entropy loss satisfy the multi-label NC. In practice, we demonstrate that our findings can lead to better test performance with more efficient training techniques for MLab learning.

==> appendices/app_exp.tex <==
% The detailed information of SVHN dataset are included in \Cref{fig:svhn_setup}
% \begin{figure}[t]
%     \centering
%     \subfloat[The SVHN Dataset]{\includegraphics[width=0.44\textwidth]{figures/SVHN_demo.png}} \
%     \hspace{0.1in}
%     \subfloat[Class Distribution]{\includegraphics[width=0.44\textwidth]{figures/svhn_mul_2_dist.png}} \
%     \caption{\textbf{Our usage of the SVHN dataset.} As illustrated in (a), the Street View House Numbers (SVHN) Dataset \citep{netzer2011reading} comprises labeled numerical characters and inherently serves as a multi-label learning dataset. We applied minimal preprocessing to achieve balance specifically within the Multiplicity-1 scenario, as evidenced by the diagonal entries in (b). Furthermore, we omitted samples with Multiplicity-4 and above, as these images posed considerable recognition challenges. Notably, the Multiplicity-2 case remained largely imbalanced, as observed in the off-diagonal entries in (b). Nonetheless, our findings remained robust and consistent in this scenario, as evidenced in \Cref{fig:NC-SVHN}.
%     }
%     \label{fig:svhn_setup}
% \end{figure}

==> appendices/app_landscape_ICML.tex <==
% \begin{theorem}[No Spurious Local Minima and Strict Saddle Property (Generalization of  \cite{zhu2021geometric}~Theorem 3.2] \label{thm:optim_landscape}
% Assume the feature dimension $d > K$, the following function 
% \begin{align} \label{eqn:loss_fn_all}
%     \min_{\mb W, \mb H, \mb b} f(\mb W, \mb H, \mb b) &= \frac{1}{Nm} \sum_{m=1}^m \sum_{i=1}^{n_m} \sum_{k=1}^{\binom{K}{m}} \mathcal{L}_{\mathtt{PAL}}( \mb{W} \mb{h}_{m,k,i} + \mb{b},  \mb{y}_{S_{m,k}}) \nonumber \\
%     & \quad + \frac{\lambda_W}{2}||\mb W||_F^2 + \frac{\lambda_H}{2} ||\mb H||_F^2 + \frac{\lambda_b}{2} ||\mb b||_2^2
% \end{align}
% with respect to $\mb W \in \mathbb{R}^{K \times d}$, $\mb H = \begin{bmatrix}
%     \mb H_1,...,\mb H_m
% \end{bmatrix} \in \mathbb{R}^{d \times Nm}$ and $\mb b \in \mathbb{R}^K$ is a strict saddle function \cite{ge2015escaping,sun2015nonconvex,zhang2020symmetry} with the following properties:
% \begin{itemize}
%     \item Any local minimizer of \cref{eqn:loss_fn_all} is a global minimizer of the form as shown in ...
%     \item Any critical point of \cref{eqn:loss_fn_all} is either a local minimum or has at least one negative curvature direction, i.e., the Hessian $\nabla^2 f(\mb W, \mb H, \mb b)$ at this point has at least one negative eigenvalue
%     \begin{align*}
%         \lambda_i (\nabla^2 f(\mb W, \mb H, \mb b)) < 0.
%     \end{align*}
% \end{itemize} 
    
% \end{theorem}


% \begin{proof}[Proof of Theorem \ref{thm:optim_landscape}]
    
% We note that the proof for Theorem 3.2 in \cite{zhu2021geometric} could be directly extended in our analysis. More specifically, the proof in \cite{zhu2021geometric} relies on a connection for the original loss function to its convex counterpart, in particular, letting $\mb Z = \mb W \mb H \in \mathbb{R}^{K \times N}$ with $N = nk$ and $\alpha=\frac{\lambda_{\mb H}}{\lambda_{\mb W}}$, the original proof first shows the following fact:
% \begin{align*}
%    \min_{\mb H\mb W = \mb Z} \; \frac{ \lambda_{\mb W} }{2} ||\mb W||_{F}^2 + \frac{ \lambda_{\mb H} }{2} ||\mb H||_{F}^2 \;&=\; \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  \min_{\mb H\mb W = \mb Z}  \;\frac{1}{2\sqrt{\alpha} } ( ||\mb W||_{F}^2 + \alpha ||\mb H||_{F}^2 ) \\
%    \;&=\; \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  ||\mb Z||_{*}.
% \end{align*}
% With the above result, the original proof relates the original loss function
% \begin{align*}
%      \min_{\mb W , \mb H,\mb b  } \; f(\mb W,\mb H,\mb b) \;:=\; g(\mb W \mb H + \mb b \mb 1^\top) \;+\; \frac{\lambda_{\mb W} }{2} ||\mb W||_{F}^2 + \frac{\lambda_{\mb H} }{2} ||\mb H||_{F}^2 + \frac{\lambda_{\mb b} }{2} ||\mb b||_{2}^2
% \end{align*}
% with 
% \begin{align*}
%     g(\mb W \mb H + \mb b \mb 1^\top) := \frac{1}{N}\sum_{k=1}^K\sum_{i=1}^n \mathcal{L}_{\mathrm{CE}}(\mb W \mb h_{k,i} + \mb b,\mb y_k),
% \end{align*}
% to a convex problem:
% \begin{align*}
%     \min_{\mb Z \in \mathbb R^{K \times N},\; \mb b \in \mathbb R^{K}}\; \widetilde{f}(\mb Z,\mb b) \;:=\; g(\mb Z + \mb b \mb 1^\top) +  \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  ||\mb Z||_{*} + \frac{\lambda_{\mb b}}{2} ||\mb b||_{2}^2.
% \end{align*}

% In our analysis, by letting $\widetilde{g}(\mb W \mb H + \mb b \mb 1^\top) := \frac{1}{Nm} \sum_{m=1}^m \sum_{i=1}^{n_m} \sum_{k=1}^{\binom{K}{m}} \mathcal{L}_{\mathtt{PAL}}( \mb{W} \mb{h}_{m,k,i} + \mb{b},  \mb{y}_{S_{m,k}})$, we can directly apply the original proof for our problem. For more details, we refer readers to the proof of Theorem 3.2 in \cite{zhu2021geometric}.
% \end{proof}


Due to the nonconvex nature of Problem \eqref{eq:DL-loss}, the characterization of global optimality alone in
\Cref{thm:GO_thm} is not sufficient for guaranteeing efficient optimization to those desired global solutions. Thus, we further study the global landscape of Problem \eqref{eq:DL-loss} by characterizing all of its critical points, we show the following result.


%In \Cref{thm:GO_thm}, we characterized the optimizers of \Cref{eq:DL-loss}. Next, we complete the analysis of this optimization problem and studying  the optimization landscape.

\begin{theorem}[\textbf{Benign Optimization Landscape}]\label{thm:landscape}
(Generalization of  \cite{zhu2021geometric}~Theorem 3.2)
    Suppose the same setting of \Cref{thm:GO_thm}, and assume the feature dimension is larger than the number of classes, i.e., $d > K$, and the number of training samples for each class are balanced within each multiplicity. Then the function $f(\bW, \bH, \bbb)$ in Problem \eqref{eq:DL-loss-ufm} is a strict saddle function with no spurious local minimum in the sense that:
%    \vspace{-0.1in}
    \begin{itemize}[leftmargin=*]
        \item Any local minimizer of $f$ is a global solution of the form described in Theorem \ref{thm:GO_thm}.
        \item Any critical point $(\bW, \bH, \mb b)$ of $f$ that is not a global minimizer is a strict saddle point with negative curvatures, in the sense that there exists some direction $(\mb \Delta_{\mb W},\mb \Delta_{\mb H}, \mb \delta_{\mb b})$ such that the directional Hessian $\nabla^2 f(\bW, \bH, \mb b)[\mb \Delta_{\mb W},\mb \Delta_{\mb H}, \mb \delta_{\mb b}]<0$. 
    \end{itemize}
\end{theorem}
%\vspace{-0.25cm}

% \begin{theorem}[No Spurious Local Minima and Strict Saddle Property (Generalization of  \cite{zhu2021geometric}~Theorem 3.2] \label{thm:optim_landscape}
% Assume the feature dimension $d > K$, the following function 
% \begin{align} \label{eqn:loss_fn_all}
%     \min_{\mb W, \mb H, \mb b} f(\mb W, \mb H, \mb b) &= \frac{1}{N} \sum_{m=1}^m \sum_{i=1}^{n_m} \sum_{k=1}^{\binom{K}{m}} \mathcal{L}_{\mathtt{PAL}}( \mb{W} \mb{h}_{m,k,i} + \mb{b},  \mb{y}_{S_{m,k}}) \nonumber \\
%     & \quad + \lambda_{\bW}||\mb W||_F^2 + \lambda_{\bH} ||\mb H||_F^2 + \lambda_{\bbb} ||\mb b||_2^2
% \end{align}
% with respect to $\mb W \in \mathbb{R}^{K \times d}$, $\mb H = \begin{bmatrix}
%     \mb H_1,...,\mb H_m
% \end{bmatrix} \in \mathbb{R}^{d \times Nm}$ and $\mb b \in \mathbb{R}^K$ is a strict saddle function \cite{ge2015escaping,sun2015nonconvex,zhang2020symmetry} with the following properties:
% \begin{itemize}
%     \item Any local minimizer of \Cref{eqn:loss_fn_all} is a global minimizer of the form as shown in \Cref{thm:GO_thm}.
%     \item Any critical point of \Cref{eqn:loss_fn_all} is either a local minimum or has at least one negative curvature direction, i.e., the Hessian $\nabla^2 f(\mb W, \mb H, \mb b)$ at this point has at least one negative eigenvalue
%     \begin{align*}
%         \lambda_i (\nabla^2 f(\mb W, \mb H, \mb b)) < 0.
%     \end{align*}
% \end{itemize} 
    
% \end{theorem}


The original proof in \cite{zhu2021geometric} connects the nonconvex optimization problem to a convex low-rank realization and then characterizes the global optimality conditions based on the convex problem. The proof concludes by analyzing all critical points, guided by the identified optimality conditions. 
Because the PAL loss for \MLab~is reduced from the CE loss in \MClf, the above result can be generalized from the result in \cite{zhu2021geometric}. 
% We defer detailed proofs to \Cref{app:landscape}.
Unlike \Cref{thm:GO_thm}, the result of benign landscape in \Cref{thm:landscape} does not hold for $d = K-1$. The reason is that we need to construct a negative curvature direction in the null space of $\bW$ for showing strict saddle points. Similar to \cite{zhu2021geometric}, we conjecture the \MLab~NC results also hold for $d = K$ and leave it for future work. 

In our paper, we establish the theoretical properties of all critical points, demonstrating that the function is a strict saddle function \cite{ge2015escaping} in the context of multi-label learning with respect to $(\bm W, \bm H)$. It's worth noting that for strict saddle functions like PAL-CE, there exists a substantial body of prior research in the literature that provides rigorous algorithmic convergence to global minimizers. In our case, this equates to achieving a global multi-label neural collapse solution. These established methods include both first-order gradient descent techniques \cite{ge2015escaping, jin2017escape, lee2019first} and second-order trust-region methods \cite{sun2016complete}, all of which ensure efficient algorithmic convergence. 

\begin{proof}[Proof of Theorem 
\ref{thm:landscape}]
%\ref{thm:optim_landscape}

    
We note that the proof for Theorem 3.2 in \cite{zhu2021geometric} could be directly extended in our analysis. More specifically, the proof in \cite{zhu2021geometric} relies on a connection for the original loss function to its convex counterpart, in particular, letting $\mb Z = \mb W \mb H \in \mathbb{R}^{K \times N}$ with $N = \sum_{m}{n_m}$ and $\alpha=\frac{\lambda_{\mb H}}{\lambda_{\mb W}}$, the original proof first shows the following fact:
\begin{align*}
   \min_{\mb H\mb W = \mb Z} \; \lambda_{\mb W} ||\mb W||_{F}^2 + \lambda_{\mb H} ||\mb H||_{F}^2 \;&=\; \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  \min_{\mb H\mb W = \mb Z}  \;\frac{1}{\sqrt{\alpha} } ( ||\mb W||_{F}^2 + \alpha ||\mb H||_{F}^2 ) \\
   \;&=\; \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  ||\mb Z||_{*}.
\end{align*}
With the above result, the original proof relates the original loss function
\begin{align*}
     \min_{\mb W , \mb H,\mb b  } \; f(\mb W,\mb H,\mb b) \;:=\; g(\mb W \mb H + \mb b \mb 1^\top) \;+\; \lambda_{\mb W} ||\mb W||_{F}^2 + \lambda_{\mb H}||\mb H||_{F}^2 + \lambda_{\mb b} ||\mb b||_{2}^2
\end{align*}
with 
\begin{align*}
    g(\mb W \mb H + \mb b \mb 1^\top) := \frac{1}{N}\sum_{k=1}^K\sum_{i=1}^n \mathcal{L}_{\mathrm{CE}}(\mb W \mb h_{k,i} + \mb b,\mb y_k),
\end{align*}
to a convex problem:
\begin{align*}
    \min_{\mb Z \in \mathbb R^{K \times N},\; \mb b \in \mathbb R^{K}}\; \widetilde{f}(\mb Z,\mb b) \;:=\; g(\mb Z + \mb b \mb 1^\top) +  \sqrt{\lambda_{\mb W} \lambda_{\mb H} }  ||\mb Z||_{*} + \lambda_{\mb b} ||\mb b||_{2}^2.
\end{align*}

In our analysis, by letting $\widetilde{g}(\mb W \mb H + \mb b \mb 1^\top) := \frac{1}{Nm} \sum_{m=1}^m \sum_{i=1}^{n_m} \sum_{k=1}^{\binom{K}{m}} \mathcal{L}_{\mathtt{PAL}}( \mb{W} \mb{h}_{m,k,i} + \mb{b},  \mb{y}_{S_{m,k}})$, we can directly apply the original proof for our problem. For more details, we refer readers to the proof of Theorem 3.2 in \cite{zhu2021geometric}.


\end{proof}

==> appendices/app_main_ICML.tex <==
\newpage 

\onecolumn
\par\noindent\rule{\textwidth}{1pt}
\begin{center}
{\Large \bf Appendix}
\end{center}
\vspace{-0.1in}
\par\noindent\rule{\textwidth}{1pt}


%\qq{we can put a table of contents here}
%\py{done}

%\makeatletter
%\setcounter{tocdepth}{3}
%\def\contentsname{Contents}
%\def\tableofcontents{%
%    \section*{\MakeUppercase{\contentsname}}%
%    \@starttoc{toc}%
%    }
%\makeatother
%\tableofcontents

%\qq{use the command of table of contents to generate}

\section*{Organization of Appendices}

\begin{table*}[h!]
\centering
\begin{tabular}{|c|clll|}
\hline
\Cref{app:related_works} & \multicolumn{4}{c|}{\textbf{Related Works and Futue Directions}}              \\ \hline
\Cref{app:data_show} & \multicolumn{4}{c|}{\textbf{Dataset Illustrations, Visualizations and Experimental Setups}} \\ \hline
\Cref{app:optimality} & \multicolumn{4}{c|}{\textbf{Proofs for Optimality Condition}}          \\ \hline
\Cref{app:landscape} & \multicolumn{4}{c|}{\textbf{Nonconvex Landscape Analysis}}             \\ \hline
\end{tabular}
\caption{\textbf{Table of Contents for Appendices}}
\end{table*}



In \Cref{app:related_works}, we provided more related work on multi-label learning and Neural Collapse with more detailed future direction of our paper. In \Cref{app:data_show}, We present all the datasets utilized for validating multi-label NC, guiding testing and training, along with the experimental setups introduced in this study. In \Cref{app:optimality}
and \Cref{app:landscape}, we present the proofs for results from the main paper \Cref{thm:GO_thm} (global optimality) and \Cref{thm:landscape} (benign landscapes), respectively. 

% \section{Dataset details}\label{app:extra-exp}
% \begin{figure}[h!]
%     \centering
%     \subfloat[MLab-MNIST]{\includegraphics[width=0.20\textwidth]{figures/mnist_0_6.eps}
%     \includegraphics[width=0.20\textwidth]{figures/mnist_3_1.eps}} \
%     ~
%     \subfloat[MLab-Cifar10]{\includegraphics[width=0.20\textwidth]{figures/c10_car_airplane.eps}
%     \includegraphics[width=0.20\textwidth]{figures/c10_dog_cat.eps}} \\
%     \caption{\textbf{Illustration of synthetic multi-label MNIST (left) and Cifar10 (right) datasets.
%     }}
%     \label{fig:sample_mnist_c10}
%     \vspace{-0.5cm}
% \end{figure}

% \input{appendices/app_exp}
% The detailed information of SVHN dataset are included in \Cref{fig:svhn_setup}
% \begin{figure}[h!]
%     \centering
%     \subfloat[The SVHN Dataset]{\includegraphics[width=0.44\textwidth]{figures/SVHN_demo.png}} \
%     \hspace{0.1in}
%     \subfloat[Class Distribution]{\includegraphics[width=0.44\textwidth]{figures/svhn_mul_2_dist.png}} \
%     \caption{\textbf{Our usage of the SVHN dataset.} As illustrated in (a), the Street View House Numbers (SVHN) Dataset \cite{netzer2011reading} comprises labeled numerical characters and inherently serves as a multi-label learning dataset. We applied minimal preprocessing to achieve balance specifically within the Multiplicity-1 scenario, as evidenced by the diagonal entries in (b). Furthermore, we omitted samples with Multiplicity-4 and above, as these images posed considerable recognition challenges. Notably, the Multiplicity-2 case remained largely imbalanced, as observed in the off-diagonal entries in (b). Nonetheless, our findings remained robust and consistent in this scenario, as evidenced in \Cref{fig:NC-SVHN}.}
%     \label{fig:svhn_setup}
% \end{figure}

\section{Related Works and Future Direction} \label{app:related_works}
\input{appendices/app_related_works}

\section{Dataset Illustration and Visualization} \label{app:data_show}
\input{appendices/app_data_show}

%\newpage
\section{Optimality Condition}\label{app:optimality}
\input{appendices/app_optimality2}

\section{Nonconvex Landscape Analysis}\label{app:landscape}

\input{appendices/app_landscape_ICML}


%\section{Future Works and Discussion}\label{app:extra_diss}

%\input{appendices/app_extra_discussion}





==> appendices/app_related_works.tex <==
\subsection{Discussion on Related Works}

\paragraph{Related works on multi-label learning.} In contrast to \MClf, where each sample has a single label, in \MLab~the samples are tagged with multiple labels. As such, the final model output must be set-valued. This presents theoretical and practical challenges unique to the regime of \MLab~learning, especially when the class number is large \cite{liu2021emerging}. 
% For \MLab, a commonly employed strategy is to decompose a given multi-label problem into several binary classification tasks \cite{menon2019multilabel}.  The ``one-versus-all'' methodology, often referred to as \emph{binary relevance} (BR), involves segmenting labels into a series of binary classification challenges. Each of these challenges necessitates the training of independent ensembles of binary classifiers, with one dedicated to each label \cite{moyano2018review, brinker2006unified}. Although BR is straightforward and able to generate good multi-hot label predictions, i.e. the prediction during inference is binary vector, not real value vector, it has faced limitations due to its oversight of label inter-dependencies \cite{cheng2010bayes}. In response to this concern, the Pick-All-Label (PAL) approach has been introduced \cite{reddi2019stochastic, menon2019multilabel}, accommodating label dependencies by treating multi-label classification as a set of parallel multi-class classification problems.
Besides BR and PAL, there are also non-decomposable approaches to \MLab~learning \cite{dembczynski2012label}. However, to the best of our knowledge, the contribution of the work \cite{dembczynski2012label} is more on the theoretical side, while it has limited impacts on training practical neural networks for \MLab. Therefore, in this work we only focus on reducible formulations such as PAL and BR. On the practical side, many modern deep neural network architectures have been successfully adapted to the multi-label task \cite{chang2020taming,lanchantin2021general,ridnik2023ml}. However, the methods often suffer from the challenges of imbalanced training data, given that high Multiplicity labels are scarce.
% Influential datasets, including ImageNet, have been re-investigated in the multi-label regime \cite{yun2021re}.

On the theory side, consistency of surrogate methods for \MLab~has been initiated by \cite{gao2011consistency} and followed up by several works in 
\cite{menon2019multilabel,dembczynski2012consistent,zhang2020convex,blondel2020learning}. Many other concepts from classical learning theory have also been extended successfully to the \MLab~regime, e.g., Vapnik-Chervonenkis theory and sample-compression schemes \cite{samei2014sample,samei2014generalizing},
(local) Rademacher complexity \cite{xu2016local,reeve2020optimistic},
and Bayes-optimal prediction \cite{cheng2010bayes}.
%However, to the best of our knowledge, no work has previously analyzed the geometric structure arisen in multi-label deep learning. Our work closes this gap, providing a generalization of the neural collapse phenomenon to multi-label learning. 


\paragraph{Related works on neural collapse.} 
The phenomenon known as NC was initially identified in recent groundbreaking research \cite{papyan2020prevalence,han2022neural} conducted on \MClf. These studies provided empirical evidence demonstrating the prevalence of NC across various network architectures and datasets. The significance of NC lies in its elegant mathematical characterization of learned representations or features in deep learning models for \MClf. Notably, this characterization is independent of network architectures, dataset properties, and optimization algorithms, as also highlighted in a recent review paper \cite{kothapalli2023neural}. Subsequent investigations, building upon the "unconstrained feature model" \cite{mixon2020neural} or the "layer-peeled model" \cite{fang2021exploring}, have contributed theoretical evidence supporting the existence of NC. This evidence pertains to the utilization of a range of loss functions, including cross-entropy (CE) loss \cite{lu2020neural,zhu2021geometric,fang2021exploring,yaras2022neural}, mean-square-error (MSE) loss \cite{mixon2020neural,zhou2022optimization,tirer2022extended,rangamani2022neural,wang2022linear,dang2023neural}, and CE variants \cite{graf2021dissecting,zhou2022all}. More recent studies have explored other theoretical aspects of NC, such as its relationship with generalization \cite{hui2022limitations,galanti2022role,galanti2022generalization,galanti2022note,chen2022perfectly}, its applicability to large classes \cite{liu2023generalizing,gao2023study,jiang2023generalized}, and the progressive collapse of feature variability across intermediate network layers \cite{hui2022limitations,papyan2020traces,he2022law,yaras2023law,rangamani2023feature}. Theoretical findings related to NC have also inspired the development of new techniques to improve practical performance in various scenarios, including the design of loss functions and architectures \cite{yu2020learning,zhu2021geometric,chan2022redunet}, transfer learning \cite{li2022principled, xie2022hidden, wang2023far} where a model trained on one task or dataset is adapted or fine-tuned to perform a different but related task, imbalanced learning \cite{fang2021exploring,xie2023neural,lu2022importance,yang2022inducing,thrampoulidis2022imbalance,behnia2023implicit,zhong2023understanding,sharma2023learning} which is a characteristic of dataset where one or more classes have significantly fewer instances compared to other classes, and continual learning \cite{yu2023continual,yang2023neural,zhai2023investigating} in which a model is designed to learn and adapt to new data continuously over time, rather than being trained on a fixed dataset. 


\subsection{Other Future Directions}

In this study, we extensively analyzed the NC phenomenon in \MLab~\cite{zhu2021geometric,fang2021exploring,ji2022unconstrained}. Based upon the UFM, our results establish that \MLab~ETFs are the only global minimizers of the PAL loss function, incorporating weight decay and bias. These findings hold significant implications for improve the performance and training efficiency of \MLab~tasks. We believe that our results open several interesting directions that is worth of further exploration that we discuss below.
%\LP{The future directions are three folds: how \MLab~NC helps improve testing performance, how \MLab~NC deals with data imbalanced-ness, and how to designed better training losses.}
%As a future direction, it would be interesting to investigate \MLab~NC to improve test performance through better designs of loss functions and regularization techniques \cite{zhou2022all}. %\LP{Our \MLab~NC also sheds light on the application of NC during testing resulting in improved testing accuracy, especially at higher multiplicities when compared to the One vs. All (OvA) approach. In future research, we would like to explore the potential of combining both One Nearest Neighbor (OneNN) and OvA techniques to create one ensemble method based on the specific multiplicity to optimize testing accuracy.} In addition, in this work we restricted our study to the case where the samples within multiplicity are balanced across different labels. For future work, an important direction is to investigate the  more challenging cases where this assumption is does not hold. A promising approach might  be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework} \cite{thrampoulidis2022imbalance}.
% \qq{expand the conclusion, discuss each bullet points in details}


\paragraph{Extreme Multi-label classification}

The goal of extreme multi-label classification is to tag a data point with the most relevant subset of labels from an extremely large label set. We have explored our \MLab~NC phenomenon on the more challenging Microsoft COCO dataset \cite{lin2014microsoft} with minimal preprocessing to maintain balance among multiplicity-1 data. The visualization of \MLab~NC measures is shown in \cref{fig:cocoNC}. Specifically, a subset of the COCO dataset comprising 32,083 samples was extracted. We included 50 classes with all higher multiplicity samples possible. Most samples belong to higher multiplicity (29,583 samples) compared to multiplicity-1 samples (only 2,500). The ResNet18 architecture was trained for 200 epochs, achieving a training IoU of around $98 \%$. For training efficiency, we fixed the classifier W as an ETF and downsampled images to 64 by 64 pixels. Under these experimental setups, we observed that $\mathcal{NC}_1$, $\mathcal{NC}_3$, and $\mathcal{NC}_m$ all converged to small values, demonstrating the Mlab-NC phenomenon.

\begin{figure*}[h]
\centering
\includegraphics[width=0.95\textwidth]{figures/coco_NCs.pdf} \    \vspace{-0.1in}
    \caption{\MLab~NC phenomenon in extreme MS-COCO dataset. As we can see that all \MLab~NC measures converges to small values.}
    \label{fig:cocoNC}
\end{figure*}

While the Microsoft COCO dataset indeed contains a large number of labels, there is still a gap between its setup and the most extreme multi-label datasets. The work by \cite{jiang2023generalized} studied the phenomenon of neural collapse under extreme multi-class classification where the number of labels exceeds the dimension of learned features. To our knowledge, no one has studied neural collapse in the context of extreme multi-label classification. Our tentative experiments on the Microsoft COCO dataset demonstrate the potential to develop a generalized neural collapse for multi-label classification with a large number of labels.


\paragraph{Features for data with all possible tags}
% While our theoretical analysis on the scaled tag-wise average property is based on the assumption that the multiplicity of a data point is smaller than total labels (i.e. $M < K$), experimental results on the toy Microsoft COCO dataset indicate that the tag-wise average property still holds for data samples with multiplicity $M = K$. The visualization of learned data features are shown in \cref{fig:toy_cocoNC_origin}. Specifically, we pick three classes: Car, Train, and Truck, where each sample can have $1-3$ labels. This means that the dataset comprises samples in mul-1, mul-2, and mul-3, based on the number of labels they carry. As we can see that both the global feature mean and the multiplicity-3 features are indeed at the origin. 

While our theoretical analysis of the scaled tag-wise average property assumes that the multiplicity of a data point is less than the total number of classes (i.e., $M<K$), experimental results on the toy Microsoft COCO dataset indicate that the tag-wise average property still holds for data samples with multiplicity $M=K$. The visualization of learned data features is shown in \cref{fig:toy_cocoNC_origin}. Specifically, we selected three classes: Car, Train, and Truck, where each sample can have $1$ to $3$ labels. This means that the dataset comprises samples with multiplicities of $1$, $2$, and $3$, based on the number of labels they carry. We then trained a 5-layer convolutional network using the selected data and we chose a feature dimension $2$ for visualization purposes. As shown in the visualization, both the global feature mean and the multiplicity-3 features are indeed located at the origin.

\begin{figure*}[h]
\centering{\includegraphics[width=0.6\textwidth]{figures/600_epoch.pdf}} \    \vspace{-0.1in}
    \caption{\MLab~NC: learned features for data samples with all possible labels is at the origin and follows tag-wise average property.}
    \label{fig:toy_cocoNC_origin}
\end{figure*}


% \begin{itemize}[leftmargin=*]
%     % \item \textbf{Improving test performance by designing better decision rules.} By reducing \MLab~to \MClf, the PAL loss considered in this work leverages the dependency and relationship between each label. Nevertheless, it is worth noting that during the testing phase, PAL yields a real-valued vector as its output, requiring extra steps for converting it into a multi-hot binary label representation. To obtain the multi-hot binary label, varying threshold levels or employing different encoding techniques are required, which yield different multi-hot labels and hence result in unpredictable testing performance. Therefore, better decision rules are needed for \MLab~learning. Based upon the observation of the \MLab~NC, we could potentially design a better threshold-free decision rule simply by using the feature nearest center. More specifically, the \MLab~NC demonstrates that features collapse to their means across all multiplicities. With this geometric understanding, a simple yet intuitive approach for encoding the predicted real value vector into a multi-hot representation for testing data is to perform a nearest class center calculation between the feature of test data and all the feature means. 
     
%     \item \textbf{Dealing with data imbalanced-ness.} As many multi-label datasets are imbalanced, another important direction is to investigate the more challenging cases where the Multiplicity-1 training data are imbalanced. We suspect a more general minority collapse phenomenon would happen \cite{fang2021exploring,thrampoulidis2022imbalance}. A promising approach might be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework}, which is related to the singular value decomposition of the simplex-encoded label matrix \cite{thrampoulidis2022imbalance}. Nonetheless, we conjecture that the scaled average property will still hold between higher multiplicity features and their multiplicity-1 features. On the other hand, when  Multiplicity-1 training data are imbalanced, it is also worth studying creating a balanced dataset through data augmentation by leveraging recent advances in diffusion models \cite{ho2020denoising,trabucco2023effective,zhang2023emergence}. 
%     % \LP{We could use diffusion model \cite{ho2020denoising} to learn the hidden distribution of the minority class in order to generate more data to create the overall balanced dataset.}

%     % \item \textbf{using diffusing model to create balanced datasets.}
    
%     \item \textbf{Designing better training loss.} Prior research has underscored the significance of mitigating within-class variability collapse to improve the transferability of learned models \cite{li2022principled}. In the context of \MLab~problems, the principle of Maximal Coding Rate Reduction (MCR$^2$) has been designed and effectively employed to foster feature diversity and discrimination, thereby preventing collapse \cite{yu2020learning,chan2022redunet}. We believe that our \MLab~NC could offer insights into the development of analogous loss functions for \MLab~learning, with the goal of promoting diversity in features.
%     %NC not welcome for transfer leanring. \MClf has MCR2 to counter act NC, further analysis needed to see if \MLab~NC is pervasive across different losses. If so, similar to MCR2, \MLab NC could be used to designed better multi-label losses that does not collapse.}
% \end{itemize}

==> arXiv_sections/conclusion.tex <==
% %xxxxxxxxxxxxxxx

% %Post-submission plan:

% In this study, we extensively analyzed the NC phenomenon in \MLab~\cite{zhu2021geometric,fang2021exploring,ji2022unconstrained}. Based upon the UFM, our results establish that \MLab~ETFs are the only global minimizers of the PAL loss function, incorporating weight decay and bias. These findings hold significant implications for improve the performance and training efficiency of \MLab~tasks. We believe that our results open several interesting directions that is worth of further exploration that we discuss below.
% %\LP{The future directions are three folds: how \MLab~NC helps improve testing performance, how \MLab~NC deals with data imbalanced-ness, and how to designed better training losses.}
% %As a future direction, it would be interesting to investigate \MLab~NC to improve test performance through better designs of loss functions and regularization techniques \cite{zhou2022all}. %\LP{Our \MLab~NC also sheds light on the application of NC during testing resulting in improved testing accuracy, especially at higher multiplicities when compared to the One vs. All (OvA) approach. In future research, we would like to explore the potential of combining both One Nearest Neighbor (OneNN) and OvA techniques to create one ensemble method based on the specific multiplicity to optimize testing accuracy.} In addition, in this work we restricted our study to the case where the samples within multiplicity are balanced across different labels. For future work, an important direction is to investigate the  more challenging cases where this assumption is does not hold. A promising approach might  be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework} \cite{thrampoulidis2022imbalance}.
% % \qq{expand the conclusion, discuss each bullet points in details}
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Improving test performance by designing better decision rules.} By reducing \MLab~to \MClf, the PAL loss considered in this work leverages the dependency and relationship between each label. Nevertheless, it is worth noting that during the testing phase, PAL yields a real-valued vector as its output, requiring extra steps for converting it into a multi-hot binary label representation. To obtain the multi-hot binary label, varying threshold levels or employing different encoding techniques are required, which yield different multi-hot labels and hence result in unpredictable testing performance. Therefore, better decision rules are needed for \MLab~learning. Based upon the observation of the \MLab~NC, we could potentially design a better threshold-free decision rule simply by using the feature nearest center. More specifically, the \MLab~NC demonstrates that features collapse to their means across all multiplicities. With this geometric understanding, a simple yet intuitive approach for encoding the predicted real value vector into a multi-hot representation for testing data is to perform a nearest class center calculation between the feature of test data and all the feature means. 
     
%     \item \textbf{Dealing with data imbalanced-ness.} As many multi-label datasets are imbalanced, another important direction is to investigate the more challenging cases where the Multiplicity-1 training data are imbalanced. We suspect a more general minority collapse phenomenon would happen \cite{fang2021exploring,thrampoulidis2022imbalance}. A promising approach might be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework}, which is related to the singular value decomposition of the simplex-encoded label matrix \cite{thrampoulidis2022imbalance}. Nonetheless, we conjecture that the scaled average property will still hold between higher multiplicity features and their multiplicity-1 features. On the other hand, when  Multiplicity-1 training data are imbalanced, it is also worth studying creating a balanced dataset through data augmentation by leveraging recent advances in diffusion models \cite{ho2020denoising,trabucco2023effective,zhang2023emergence}. 
%     % \LP{We could use diffusion model \cite{ho2020denoising} to learn the hidden distribution of the minority class in order to generate more data to create the overall balanced dataset.}

%     % \item \textbf{using diffusing model to create balanced datasets.}
    
%     \item \textbf{Designing better training loss.} Prior research has underscored the significance of mitigating within-class variability collapse to improve the transferability of learned models \cite{li2022principled}. In the context of \MLab problems, the principle of Maximal Coding Rate Reduction (MCR$^2$) has been designed and effectively employed to foster feature diversity and discrimination, thereby preventing collapse \cite{yu2020learning,chan2022redunet}. We believe that our \MLab~NC could offer insights into the development of analogous loss functions for \MLab learning, with the goal of promoting diversity in features.
%     %NC not welcome for transfer leanring. \MClf has MCR2 to counter act NC, further analysis needed to see if \MLab~NC is pervasive across different losses. If so, similar to MCR2, \MLab NC could be used to designed better multi-label losses that does not collapse.}
% \end{itemize}




% %Furthermore, an interesting direction for expanding our work on multi-label data learning is to the imbalanced setting \cite{thrampoulidis2022imbalance}. Exploring this area would also involve investigating the effects of 

In this study, we extensively analyzed the NC phenomenon in \MLab~\cite{zhu2021geometric,fang2021exploring,ji2022unconstrained}. Based upon the UFM, our results establish that \MLab~ETFs are the only global minimizers of the PAL loss function, incorporating weight decay and bias. These findings hold significant implications for improve the performance and training efficiency of \MLab~tasks. We believe that our results open several interesting directions that is worth of further exploration that we discuss below.
%\LP{The future directions are three folds: how \MLab~NC helps improve testing performance, how \MLab~NC deals with data imbalanced-ness, and how to designed better training losses.}
%As a future direction, it would be interesting to investigate \MLab~NC to improve test performance through better designs of loss functions and regularization techniques \cite{zhou2022all}. %\LP{Our \MLab~NC also sheds light on the application of NC during testing resulting in improved testing accuracy, especially at higher multiplicities when compared to the One vs. All (OvA) approach. In future research, we would like to explore the potential of combining both One Nearest Neighbor (OneNN) and OvA techniques to create one ensemble method based on the specific multiplicity to optimize testing accuracy.} In addition, in this work we restricted our study to the case where the samples within multiplicity are balanced across different labels. For future work, an important direction is to investigate the  more challenging cases where this assumption is does not hold. A promising approach might  be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework} \cite{thrampoulidis2022imbalance}.
% \qq{expand the conclusion, discuss each bullet points in details}
\begin{itemize}[leftmargin=*]
    % \item \textbf{Improving test performance by designing better decision rules.} By reducing \MLab~to \MClf, the PAL loss considered in this work leverages the dependency and relationship between each label. Nevertheless, it is worth noting that during the testing phase, PAL yields a real-valued vector as its output, requiring extra steps for converting it into a multi-hot binary label representation. To obtain the multi-hot binary label, varying threshold levels or employing different encoding techniques are required, which yield different multi-hot labels and hence result in unpredictable testing performance. Therefore, better decision rules are needed for \MLab~learning. Based upon the observation of the \MLab~NC, we could potentially design a better threshold-free decision rule simply by using the feature nearest center. More specifically, the \MLab~NC demonstrates that features collapse to their means across all multiplicities. With this geometric understanding, a simple yet intuitive approach for encoding the predicted real value vector into a multi-hot representation for testing data is to perform a nearest class center calculation between the feature of test data and all the feature means. 
     
    \item \textbf{Dealing with data imbalanced-ness.} As many multi-label datasets are imbalanced, another important direction is to investigate the more challenging cases where the Multiplicity-1 training data are imbalanced. We suspect a more general minority collapse phenomenon would happen \cite{fang2021exploring,thrampoulidis2022imbalance}. A promising approach might be employing the \emph{Simplex-Encoded-Labels Interpolation (SELI) framework}, which is related to the singular value decomposition of the simplex-encoded label matrix \cite{thrampoulidis2022imbalance}. Nonetheless, we conjecture that the scaled average property will still hold between higher multiplicity features and their multiplicity-1 features. On the other hand, when  Multiplicity-1 training data are imbalanced, it is also worth studying creating a balanced dataset through data augmentation by leveraging recent advances in diffusion models \cite{ho2020denoising,trabucco2023effective,zhang2023emergence}. 
    % \LP{We could use diffusion model \cite{ho2020denoising} to learn the hidden distribution of the minority class in order to generate more data to create the overall balanced dataset.}

    % \item \textbf{using diffusing model to create balanced datasets.}
    
    \item \textbf{Designing better training loss.} Prior research has underscored the significance of mitigating within-class variability collapse to improve the transferability of learned models \cite{li2022principled}. In the context of \MLab problems, the principle of Maximal Coding Rate Reduction (MCR$^2$) has been designed and effectively employed to foster feature diversity and discrimination, thereby preventing collapse \cite{yu2020learning,chan2022redunet}. We believe that our \MLab~NC could offer insights into the development of analogous loss functions for \MLab learning, with the goal of promoting diversity in features.
    %NC not welcome for transfer leanring. \MClf has MCR2 to counter act NC, further analysis needed to see if \MLab~NC is pervasive across different losses. If so, similar to MCR2, \MLab NC could be used to designed better multi-label losses that does not collapse.}
\end{itemize}

==> arXiv_sections/reproductivity.tex <==
The complete proof of \Cref{thm:GO_thm} and \Cref{thm:landscape} are shown in \Cref{app:optimality} and \Cref{app:landscape} respectively. Our code is available in the supplementary materiel.


==> macro.tex <==

\usepackage{url}
%\usepackage[hidelinks]{hyperref}
\usepackage{amsmath,amsthm,amssymb,amsbsy,amsfonts,amscd,bm}
\usepackage{paralist}
\usepackage{xcolor}
\usepackage{color}
\usepackage{graphicx}
\graphicspath{{./figs/}}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{comment}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fancyhdr}
%\usepackage{cite}
%\usepackage{citesort}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage[toc, page]{appendix}
% Theorems
\def \remarks {\noindent {\bf Remarks.}\ \ }
\newtheorem{thm}{Theorem}%[section] %(If you want theorem numbered
%\newtheorem{lemma}{Lemma}%[section] %%    with section number.
\newtheorem{cor}{Corollary}%[section]
\newtheorem{prop}{Proposition}%[section]
%\newtheorem{definition}{Definition}%[section]
\newtheorem{defi}{Definition}%[section]
\newtheorem{assum}{Assumption}
\newtheorem*{goal}{Plan}
%\newtheorem{theorem}{Theorem}
\newtheorem{lem}{Lemma}
\theoremstyle{remark}
%\newtheorem{remark}{Remark}
%\theoremstyle{problem}
\newtheorem{problem}{Problem}

% fields
\renewcommand{\O}{\mathbb{O}}
\newcommand{\R}{\mathbb{R}}
\def \real    { \mathbb{R} }
\def \reals   { \mathbb{R} }
\def \Real {\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\def \complex{\mathbb{C}}
\def \Complex {\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

%%%
\newcommand{\xiao}[1]{{\color{magenta}{\bf Xiao: #1}}}
%%%
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}
\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\en}{\begin{equation*}}
\newcommand{\een}{\end{equation*}}
\newcommand{\eqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bmat}{\begin{bmatrix}}
\newcommand{\emat}{\end{bmatrix}}
% complex numbers
\renewcommand{\Re}[1]{\operatorname{Re}\left\{#1\right\}}
\renewcommand{\Im}[1]{\operatorname{Im}\left\{#1\right\}}
\newcommand{\conj}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
% probability and stat
\renewcommand{\P}[1]{\operatorname{\mathbb{P}}\left(#1\right)}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\dif}{\operatorname{d}}
\newcommand{\var}{\operatorname{var}}

% calculus
\renewcommand{\d}[1]{\,\mathrm{d}#1}

% constants (written in roman, if wanted)
%\newcommand{\e}{\mathrm{e}}
\renewcommand{\j}{\mathrm{j}}

\newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
\newcommand{ \brac }[1]{\left[ #1 \right]}
%\newcommand{ \paren }[1]{ \left( #1 \right) }



\newcommand{\mb}{\bm}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\bb}{\mathbb}
\newcommand{\mrm}{\mathrm}
\newcommand{\mtt}{\mathtt}
\def \vecword  {\operatorname*{vec}}
% linear algebra
% 	vector notation
\newcommand{\vct}[1]{\boldsymbol{#1}}
%   matrices
\newcommand{\mtx}[1]{\boldsymbol{#1}}
%   block vector
\newcommand{\bvct}[1]{\mathbf{#1}}
%   block matrix
\newcommand{\bmtx}[1]{\mathbf{#1}}
%	inner products
\newcommand{\inner}[1]{\left<#1\right>}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
% 	transpose, Hermitian, pseudo-inverse
\renewcommand{\H}{\mathrm{H}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\pinv}{\dagger}
%	fundamental subspaces
\newcommand{\Null}{\operatorname{Null}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\Span}{\operatorname{Span}}
%	operators
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\toep}{\operatorname{Toep}}
\newcommand{\SDP}{\operatorname{SDP}}
\newcommand{\PSD}{\operatorname{PSD}}
\newcommand{\far}{\operatorname{far}}
\newcommand{\near}{\operatorname{near}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sign}{\operatorname{Sgn}}
\newcommand{\dist}{\operatorname{dist}}
\def \lg        {\langle}
\def \rg        {\rangle}
\def \vec       {\operatorname*{vec}}
%
\newcommand{\dimension}{\operatorname{dim}}

% sets and topology
\newcommand{\set}[1]{\mathbb{#1}}
\newcommand{\closure}{\operatorname{cl}}	% closure
\newcommand{\interior}{\operatorname{int}}
\newcommand{\boundary}{\operatorname{bd}}
\newcommand{\diameter}{\operatorname{diam}}

% functional analysis
\newcommand{\domain}{\operatorname{dom}}
\newcommand{\epigraph}{\operatorname{epi}}
\newcommand{\hypograph}{\operatorname{hypo}}
\newcommand{\linop}[1]{\mathscr{#1}}	% general linear operator

% optimization
\DeclareMathOperator*{\minimize}{\text{minimize}}
\DeclareMathOperator*{\maximize}{\text{maximize}}
\DeclareMathOperator*{\argmin}{\text{arg~min}}
\DeclareMathOperator*{\argmax}{\text{arg~max}}
%\def \st {\operatorname*{s.t.\ }}
% other
%\newcommand{\sgn}{\text{sgn}}
\newcommand{\sinc}{\text{sinc}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\eps}{\epsilon}


\newcommand{\wh}{\widehat}
\newcommand{\wc}{\widecheck}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}


\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\nrm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\parans}[1]{\left(#1\right)}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right)}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}
\newcommand{\iter}[1]{^{(#1)}}


\newcommand{\js}[1]{{\color{Mahogany} [\noindent JS: #1]}}

%--------------------------------------------------------------------------
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\hypersetup{
    colorlinks=true,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}

% \newcommand{ \Brac }[1]{\left\lbrace #1 \right\rbrace}
% \newcommand{ \brac }[1]{\left[ #1 \right]}
\newcommand{ \paren }[1]{ \left( #1 \right) }

\newcommand{\NC}{$\mc {NC}$}

\newcommand{\va}{\vct{a}}
\newcommand{\vb}{\vct{b}}
\newcommand{\vc}{\vct{c}}
\newcommand{\vd}{\vct{d}}
\newcommand{\ve}{\vct{e}}
\newcommand{\vf}{\vct{f}}
\newcommand{\vg}{\vct{g}}
\newcommand{\vh}{\vct{h}}
\newcommand{\vi}{\vct{i}}
\newcommand{\vj}{\vct{j}}
\newcommand{\vk}{\vct{k}}
\newcommand{\vl}{\vct{l}}
\newcommand{\vm}{\vct{m}}
\newcommand{\vn}{\vct{n}}
\newcommand{\vo}{\vct{o}}
\newcommand{\vp}{\vct{p}}
\newcommand{\vq}{\vct{q}}
\newcommand{\vr}{\vct{r}}
\newcommand{\vs}{\vct{s}}
\newcommand{\vt}{\vct{t}}
\newcommand{\vu}{\vct{u}}
\newcommand{\vv}{\vct{v}}
\newcommand{\vw}{\vct{w}}
\newcommand{\vx}{\vct{x}}
\newcommand{\vy}{\vct{y}}
\newcommand{\vz}{\vct{z}}
%
\newcommand{\valpha}{\vct{\alpha}}
\newcommand{\vbeta}{\vct{\beta}}
\newcommand{\vtheta}{\vct{\theta}}
\newcommand{\vepsilon}{\vct{\epsilon}}
\newcommand{\veps}{\vct{\epsilon}}
\newcommand{\vvarepsilon}{\vct{\varepsilon}}
\newcommand{\vgamma}{\vct{\gamma}}
\newcommand{\vlambda}{\vct{\lambda}}
\newcommand{\vnu}{\vct{\nu}}
\newcommand{\vphi}{\vct{\phi}}
\newcommand{\vpsi}{\vct{\psi}}
\newcommand{\vdelta}{\vct{\delta}}
\newcommand{\veta}{\vct{\eta}}
\newcommand{\vxi}{\vct{\xi}}
\newcommand{\vmu}{\vct{\mu}}
\newcommand{\vrho}{\vct{\rho}}
%
\newcommand{\vzero}{\vct{0}}
\newcommand{\vone}{\vct{1}}


\newcommand{\mA}{\mtx{A}}
\newcommand{\mB}{\mtx{B}}
\newcommand{\mC}{\mtx{C}}
\newcommand{\mD}{\mtx{D}}
\newcommand{\mE}{\mtx{E}}
\newcommand{\mF}{\mtx{F}}
\newcommand{\mG}{\mtx{G}}
\newcommand{\mH}{\mtx{H}}
\newcommand{\mJ}{\mtx{J}}
\newcommand{\mK}{\mtx{K}}
\newcommand{\mL}{\mtx{L}}
\newcommand{\mM}{\mtx{M}}
\newcommand{\mN}{\mtx{N}}
\newcommand{\mO}{\mtx{O}}
\newcommand{\mP}{\mtx{P}}
\newcommand{\mQ}{\mtx{Q}}
\newcommand{\mR}{\mtx{R}}
\newcommand{\mS}{\mtx{S}}
\newcommand{\mT}{\mtx{T}}
\newcommand{\mU}{\mtx{U}}
\newcommand{\mV}{\mtx{V}}
\newcommand{\mW}{\mtx{W}}
\newcommand{\mX}{\mtx{X}}
\newcommand{\mY}{\mtx{Y}}
\newcommand{\mZ}{\mtx{Z}}
%
\newcommand{\mGamma}{\mtx{\Gamma}}
\newcommand{\mDelta}{\mtx{\Delta}}
\newcommand{\mLambda}{\mtx{\Lambda}}
\newcommand{\mOmega}{\mtx{\Omega}}
\newcommand{\mPhi}{\mtx{\Phi}}
\newcommand{\mPsi}{\mtx{\Psi}}
\newcommand{\mSigma}{\mtx{\Sigma}}
\newcommand{\mTheta}{\mtx{\Theta}}
\newcommand{\mUpsilon}{\mtx{\Upsilon}}
%
\newcommand{\mId}{\bmtx{I}}
\newcommand{\mEx}{{\bf J}}
\newcommand{\mzero}{{\bf 0}}
\newcommand{\mone}{{\bf 1}}
%
\newcommand{\bva}{\bvct{a}}
\newcommand{\bvh}{\bvct{h}}
\newcommand{\bvw}{\bvct{w}}
\newcommand{\bvx}{\bvct{x}}
\newcommand{\bvy}{\bvct{y}}


\newcommand{\bmM}{\bmtx{M}}
\newcommand{\bmH}{\bmtx{H}}
\newcommand{\bmX}{\bmtx{X}}


\newcommand{\setA}{\set{A}}
\newcommand{\setB}{\set{B}}
\newcommand{\setC}{\set{C}}
\newcommand{\setD}{\set{D}}
\newcommand{\setE}{\set{E}}
\newcommand{\setF}{\set{F}}
\newcommand{\setG}{\set{G}}
\newcommand{\setH}{\set{H}}
\newcommand{\setI}{\set{I}}
\newcommand{\setJ}{\set{J}}
\newcommand{\setK}{\set{K}}
\newcommand{\setL}{\set{L}}
\newcommand{\setM}{\set{M}}
\newcommand{\setN}{\set{N}}
\newcommand{\setO}{\set{O}}
\newcommand{\setP}{\set{P}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setR}{\set{R}}
\newcommand{\setS}{\set{S}}
\newcommand{\setT}{\set{T}}
\newcommand{\setU}{\set{U}}
\newcommand{\setV}{\set{V}}
\newcommand{\setW}{\set{W}}
\newcommand{\setX}{\set{X}}
\newcommand{\setY}{\set{Y}}
\newcommand{\setZ}{\set{Z}}

\renewcommand{\ss}{{\vspace*{-1mm}}}

\setcounter{MaxMatrixCols}{20}

%\pagestyle{plain}

\graphicspath{{./figs/}}

\newlength{\imgwidth}
\setlength{\imgwidth}{3.125in}

\newcommand{\QW}[1]{\textcolor{red}{\bf [{\em QW:} #1]}}
\newcommand{\note}[1]{\textcolor{blue}{\bf [{\em Note:} #1]}}
\newcommand{\revise}[1]{\textcolor{blue}{#1}}
\newcommand{\edit}[1]{\textcolor{blue}{#1}}

\newboolean{twoColVersion}
\setboolean{twoColVersion}{false}
\newcommand{\twoCol}[2]{\ifthenelse{\boolean{twoColVersion}} {#1} {#2} }


\newcommand{\Poff}{\mathcal{P}_{\textup{off}}}
\newcommand{\Pon}{\mathcal{P}_{\textup{diag}}}

\newcommand{\cy}[1]{\textcolor{red}{\bf [{\em Can:} #1]}}
\newcommand{\qq}[1]{\textcolor{blue}{\bf [{\em Qing:} #1]}}
\newcommand{\yw}[1]{\textcolor{purple}{\bf [{\em Yutong:} #1]}}
\newcommand{\py}[1]{\textcolor{orange}{[#1]}}
\newcommand{\pw}[1]{\textcolor{red}{\bf [{\em Peng:} #1]}}
\newcommand{\zz}[1]{\textcolor{blue}{ [{\em Zhihui:} #1]}}
\newcommand{\jz}[1]{\textcolor{red}{ [{\em Jinxin:} #1]}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}


%\newcommand{\calL}{\mathcal{L}}
\newcommand{\act}{\sigma}
\newcommand{\PrecAt}{\mathtt{Prec}\mbox{@}}

\newcommand{\pow}{\mathcal{P}}

% macros.tex
% useful macros (shortcuts) to save typing; add more as needed!

%\newtheorem{proposition}{\bf{Proposition}}
%\newtheorem{remark}{\bf{Remark}}
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}

% now define useful macros

\long\def\comment#1{}
\newcommand{\fref}[1] {Fig.~\ref{#1}\xspace}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\Expi}[1]{\mathrm{e}^{\imath #1}}
\newcommand{\xtrue}{\xmath{\x_{\text{true}}}}
\newcommand{\cdft}{\xmath{c_{\text{dft}}}}
%\newcommand{\argmin}{\operatorname{argmin}\ }
%\newcommand{\diag}{\operatorname{diag}}
\newcommand{\tr}{\operatorname{tr}}
%\newcommand{\st}{\operatorname{s.t.}}
\newcommand{\range}{\operatorname{Range}}
%\newcommand{\rank}{\operatorname{rank}}
\renewcommand{\dim}{\operatorname{dim}}
\newcommand{\pri}{\text{pri}}
\newcommand{\dual}{\text{dual}}
\newcommand{\etal}{\textit{et al. }}
%\newcommand{\bmat}[1] {\begin{bmatrix} #1 \end{bmatrix}} % best arrays ever

\newcommand{\xmath}[1] {\ensuremath{#1}\xspace}
\newcommand{\blmath}[1] {\xmath{\bm{#1}}}
\newcommand{\A}{\blmath{A}}
\newcommand{\B}{\blmath{B}}
%\newcommand{\C}{\blmath{C}}
\newcommand{\D}{\blmath{D}}
%\newcommand{\E}{\blmath{E}}
\newcommand{\F}{\blmath{F}}
\newcommand{\I}{\blmath{I}}
%\newcommand{\R}{\blmath{R}}
%\newcommand{\T}{\blmath{T}}
\newcommand{\U}{\blmath{U}}
\newcommand{\V}{\blmath{V}}
\newcommand{\W}{\blmath{W}}
\newcommand{\X}{\blmath{X}}
\newcommand{\Y}{\blmath{Y}}
%\newcommand{\Z}{\blmath{Z}}

\newcommand{\x}{\blmath{x}}
\newcommand{\s}{\blmath{s}}
\newcommand{\y}{\blmath{y}}
\newcommand{\z}{\blmath{z}}
\newcommand{\1}{\blmath{1}} 
\newcommand{\0}{\blmath{0}} 
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\ie}{\text{i.e.}}
\newcommand{\eg}{\text{e.g.}}

\newcommand{\bLam}{\blmath{\Lambda}}


\let\originalu\u
\let\originalv\v

\newcommand{\bi} {\xmath{b_i}}
\newcommand{\hi} {\xmath{h_i}}
\newcommand{\dhi} {\xmath{\dot h_i}}
\newcommand{\ddhi} {\xmath{\ddot h_i}}
\newcommand{\ti} {\xmath{t_i}}
\newcommand{\ui} {\xmath{u_i}}
%\newcommand{\vi} {\xmath{v_i}}
\newcommand{\yi} {\xmath{y_i}}

\newcommand{\defequ} {\triangleq}
\newcommand{\sumi} {\xmath{\sum_i \; }}
\newcommand{\Wmax}{\xmath{\W_{\max}}}
\newcommand{\Wimp}{\blmath{W}_{\mathrm{imp}}}
%\newcommand{\real}[1] {\mathrm{real}\!\left\{#1\right\}}
%\newcommand{\sign}[1] {\mathrm{sign}\!\left(#1\right)}
%\newcommand{\abs}[1] {\left| #1 \right|}
\newcommand{\absb}[1] {\big| #1 \big|}
\newcommand{\Half} {\frac{1}{2}}

\newcommand{\notezl}[1] {\textcolor{red}{ZL: #1}}

%\newcommand{\reals} {\xmath{\mathbb{R}}}
%\newcommand{\complex} {\xmath{\mathbb{C}}}
\newcommand{\RM} {\xmath{\reals^M}}
\newcommand{\CN} {\xmath{\complex^N}}
\newcommand{\baih} {\xmath{\ba_i'}}
\newcommand{\psii} {\xmath{\psi_i}}
\newcommand{\bpsi} {\blmath{\psi}}

\newcommand{\Ah} {\xmath{\A'}}

\newcommand{\xk} {\xmath{\blmath{x}_k}}
\newcommand{\xkk} {\xmath{\blmath{x}_{k+1}}}
\newcommand{\zkk} {\xmath{\blmath{z}_{k+1}}}
\newcommand{\dk} {\xmath{\blmath{d}_k}}
%\newcommand{\vk} {\xmath{\blmath{v}_k}}
\newcommand{\vkk} {\xmath{\blmath{v}_{k+1}}}
\renewcommand{\u} {\blmath{u}}
\renewcommand{\v} {\blmath{v}}

\newcommand{\figref}[2] {Fig.~\ref{#1}}
\newcommand{\figcap}[3] { % file width caption
\begin{figure}
    \centering
    \includegraphics[width=#2\linewidth]{fig/#1}
    \caption{#3}
    \label{fig:#1}
\end{figure}
}

% KL below here

%\newcommand{\qed}{\hfill\rule{2mm}{2mm}}
\newcommand{\svskip}{\vspace{1.75mm}}
\newcommand{\mvskip}{\vspace{.25in}}
\newcommand{\lvskip}{\vspace{.5in}}
\def\E{\mathop{\rm E\,\!}\nolimits}
\def\Var{\mathop{\rm Var}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\den{\mathop{\rm den}\nolimits}
\def\midd{\mathop{\,|\,}\nolimits}
\def\sgn{\mathop{\rm sgn}\nolimits}
\def\vec{\mathop{\rm vec}\nolimits}
\def\sinc{\mathop{\rm sinc}\nolimits}
\def\curl{\mathop{\rm curl}\nolimits}
\def\div{\mathop{\rm div}\nolimits}
\def\tr{\mathop{\rm tr}\nolimits}
\def\len{\mathop{\rm len}\nolimits}
%\def\diag{\mathop{\rm diag}\nolimits}
\def\dist{\mathop{\rm dist}\nolimits}
\def\amp{\mathop{\;\:}\nolimits}

\newcommand{\ba}{\boldsymbol{a}}

\newcommand{\bbb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bff}{\boldsymbol{f}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}
%\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bk}{\boldsymbol{k}}
\newcommand{\bl}{\boldsymbol{l}}
%\newcommand{\bm}{\boldsymbol{m}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bo}{\boldsymbol{o}}
\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}


\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bleta}{\boldsymbol{\eta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btheta}{\xmath{\bm{\theta}}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}

\def\b{{\blmath b}} 
\def\L{{\cal L}}
%\newcommand{\paren}[1]{\left( #1 \right)}
\long\def\red#1{\bgroup\color{red}#1\egroup}

\newcommand{\of}[1]{\!\paren{#1}}
\newcommand{\dH} {\xmath{\dot{H}}}
\newcommand{\Xs} {\xmath{\mathcal{X}_s}}
\newcommand{\Lip} {\xmath{\mathcal{L}}}
\newcommand{\copt}{\xmath{c_{\mathrm{opt}}}}
\newcommand{\cimp}{\xmath{c_{\text{imp}}}}
%\newcommand{\todo}[1]{\textbf{Todo: #1}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\ith}{i^{\mathrm{th}}}


\definecolor{mich-blue}{HTML}{0027CC}
\definecolor{mich-blue-high}{HTML}{0027CC}
%\definecolor{mich-blue}{HTML}{00274C}
%\definecolor{mich-blue-high}{HTML}{00408C}
\definecolor{red-high}{HTML}{CA2020}
\definecolor{green-high}{HTML}{20A520}
\definecolor{mich-maize}{HTML}{FFCB05}
\definecolor{law-stone}{HTML}{655A52}
\definecolor{burton-beige}{HTML}{9B9A9D}
\definecolor{arch-ivy}{HTML}{7E732F}

\newcommand{\highlight}[1]{\textcolor{mich-blue-high}{#1}} 
\newcommand{\highlightred}[1]{\textcolor{red-high}{#1}} 
\newcommand{\highlightgreen}[1]{\textcolor{green-high}{#1}} \colorlet{color1}{gray!15}
\newcommand{\hlnew}[1]{\highlight{\colorbox{color1}{#1}}}
\newcommand{\xtz} {\xmath{\tilde{\blmath{x}}_0}}
\newcommand{\fF}{\xmath{\mathbb{F}}}
\newcommand{\eE}{\xmath{\mathbb{E}}}
\newcommand{\FN}{\xmath{\fF^N}}
\newcommand{\FNN}{\xmath{\fF^{N\times N}}}
\newcommand{\subdot}{_{\bm{\cdot}}}


\newcommand{\MLab}{{M-lab}}
\newcommand{\MClf}{{M-clf}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

